Generalized cluster algorithms for Potts lattice gauge theory

Monte Carlo algorithms, like the Swendsen-Wang and invaded-cluster, sample the Ising and Potts models asymptotically faster than single-spin Glauber dynamics do. Here, we generalize both algorithms to sample Potts lattice gauge theory by way of a $2$-dimensional cellular representation called the plaquette random-cluster model. The invaded-cluster algorithm targets Potts lattice gauge theory at criticality by implementing a stopping condition defined in terms of homological percolation, the emergence of spanning surfaces on the torus. Simulations for $\mathbb Z(2)$ and $\mathbb Z(3)$ lattice gauge theories on the cubical $4$-dimensional torus indicate that both generalized algorithms exhibit much faster autocorrelation decay than single-spin dynamics and allow for efficient sampling on $4$-dimensional tori of linear scale at least $40$.

==> tables/InvadedCluster.Persistence.2.tex <==


\begin{tabular}{cccc}
 &  &  & \textbf{s/it} \\
$N$ & \textbf{Plaq} & \textbf{Field} &  \\
\multirow[c]{4}{*}{256} & \multirow[c]{4}{*}{131,072} & $\mathbb Z_2$ & 0.237 \\
 &  & $\mathbb Z_3$ & 12.595 \\
 &  & $\mathbb Z_5$ & 8.843 \\
 &  & $\mathbb Z_7$ & 7.768 \\
\cline{1-4} \cline{2-4}
\multirow[c]{4}{*}{512} & \multirow[c]{4}{*}{524,288} & $\mathbb Z_2$ & 1.105 \\
 &  & $\mathbb Z_3$ & 145.532 \\
 &  & $\mathbb Z_5$ & 76.667 \\
 &  & $\mathbb Z_7$ & 62.254 \\
\cline{1-4} \cline{2-4}
\end{tabular}


==> tables/InvadedCluster.Persistence.4.tex <==


\begin{tabular}{cccc}
 &  &  & \textbf{s/it} \\
$N$ & \textbf{Plaq} & \textbf{Field} &  \\
\multirow[c]{2}{*}{10} & \multirow[c]{2}{*}{60,000} & $\mathbb Z_2$ & 0.847 \\
 &  & $\mathbb Z_3$ & 42.541 \\
\cline{1-4} \cline{2-4}
\end{tabular}


==> tables/SwendsenWang.ReducedKernelSample.2.tex <==


\begin{tabular}{cccc}
 &  &  & \textbf{s/it} \\
$N$ & \textbf{Plaq} & \textbf{Field} &  \\
\multirow[c]{4}{*}{256} & \multirow[c]{4}{*}{131,072} & $\mathbb Z_2$ & 0.253 \\
 &  & $\mathbb Z_3$ & 0.177 \\
 &  & $\mathbb Z_5$ & 0.119 \\
 &  & $\mathbb Z_7$ & 0.102 \\
\cline{1-4} \cline{2-4}
\multirow[c]{4}{*}{512} & \multirow[c]{4}{*}{524,288} & $\mathbb Z_2$ & 1.286 \\
 &  & $\mathbb Z_3$ & 0.702 \\
 &  & $\mathbb Z_5$ & 0.431 \\
 &  & $\mathbb Z_7$ & 0.353 \\
\cline{1-4} \cline{2-4}
\multirow[c]{4}{*}{1024} & \multirow[c]{4}{*}{2,097,152} & $\mathbb Z_2$ & 7.135 \\
 &  & $\mathbb Z_3$ & 3.698 \\
 &  & $\mathbb Z_5$ & 2.038 \\
 &  & $\mathbb Z_7$ & 1.605 \\
\cline{1-4} \cline{2-4}
\multirow[c]{4}{*}{2048} & \multirow[c]{4}{*}{8,388,608} & $\mathbb Z_2$ & 67.837 \\
 &  & $\mathbb Z_3$ & 28.235 \\
 &  & $\mathbb Z_5$ & 11.285 \\
 &  & $\mathbb Z_7$ & 7.813 \\
\cline{1-4} \cline{2-4}
\end{tabular}


==> tables/SwendsenWang.ReducedKernelSample.4.tex <==


\begin{tabular}{cccc}
 &  &  & \textbf{s/it} \\
$N$ & \textbf{Plaq} & \textbf{Field} &  \\
\multirow[c]{4}{*}{10} & \multirow[c]{4}{*}{60,000} & $\mathbb Z_2$ & 0.206 \\
 &  & $\mathbb Z_3$ & 0.132 \\
 &  & $\mathbb Z_5$ & 0.093 \\
 &  & $\mathbb Z_7$ & 0.091 \\
\cline{1-4} \cline{2-4}
\multirow[c]{4}{*}{20} & \multirow[c]{4}{*}{960,000} & $\mathbb Z_2$ & 3.161 \\
 &  & $\mathbb Z_3$ & 1.683 \\
 &  & $\mathbb Z_5$ & 1.076 \\
 &  & $\mathbb Z_7$ & 0.888 \\
\cline{1-4} \cline{2-4}
\multirow[c]{4}{*}{30} & \multirow[c]{4}{*}{4,860,000} & $\mathbb Z_2$ & 28.550 \\
 &  & $\mathbb Z_3$ & 12.539 \\
 &  & $\mathbb Z_5$ & 6.381 \\
 &  & $\mathbb Z_7$ & 5.234 \\
\cline{1-4} \cline{2-4}
\multirow[c]{4}{*}{40} & \multirow[c]{4}{*}{15,360,000} & $\mathbb Z_2$ & 224.594 \\
 &  & $\mathbb Z_3$ & 79.565 \\
 &  & $\mathbb Z_5$ & 27.017 \\
 &  & $\mathbb Z_7$ & 19.159 \\
\cline{1-4} \cline{2-4}
\end{tabular}

